Interacting Particle Markov Chain Monte Carlo

We introduce interacting particle Markov chain Monte Carlo (iPMCMC), a PMCMC method based on an interacting pool of standard and conditional sequential Monte Carlo samplers. Like related methods, iPMCMC is a Markov chain Monte Carlo sampler on an extended space. We present empirical results that show significant improvements in mixing rates relative to both non-interacting PMCMC samplers, and a single PMCMC sampler with an equivalent memory and computational budget. An additional advantage of the iPMCMC method is that it is suitable for distributed and multi-core architectures.

==> algorithm.tex <==
\tikzstyle{smc}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=blue!80,
                                    fill=blue!40]
\tikzstyle{csmc}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=red!80,
                                    fill=red!20]

\tikzstyle{background}=[rectangle,
                                                fill=gray!10,
                                                inner sep=0.2cm,
                                                rounded corners=5mm]

\begin{tikzpicture}[>=latex,text height=1.5ex,text depth=0.25ex]
  \matrix[row sep=0.5cm,column sep=0.5cm] {
    %&
        \node (j) []{$m$};           &
        \node (j1) []{$\mathbf{1}$}; &
        \node (j2) []{$\mathbf{2}$}; &
        \node (j3) []{$\mathbf{3}$}; &
        \node (j4) []{$\mathbf{4}$}; &
        \node (j5) []{$\mathbf{5}$}; &
        \\
        &
        \node (d1) []{$\vdots$}; &
        \node (d2) []{$\vdots$}; &
        \node (d3) []{$\vdots$}; &
        \node (d4) []{$\vdots$}; &
        \node (d5) []{$\vdots$}; &
        \\
        \node (r-1) []{$r-1$};      &
        \node (r-1_1) [smc]{};      &
        \node (r-1_2) [smc]{};      &
        \node (r-1_3) [csmc]{};     &
        \node (r-1_4) [smc]{};      &
        \node (r-1_5) [csmc]{};     &
        \\
        \node (r) []{$r$};          &
        \node (r_1) [smc]{};        &
        \node (r_2) [csmc]{};       &
        \node (r_3) [smc]{};        &
        \node (r_4) [smc]{};        &
        \node (r_5) [csmc]{};       &
        \\
        \node (r+1) []{$r+1$};      &
        \node (r+1_1) [smc]{};      &
        \node (r+1_2) [csmc]{};     &
        \node (r+1_3) [smc]{};      &
        \node (r+1_4) [smc]{};      &
        \node (r+1_5) [csmc]{};     &
        \\
        &
        \node (d21) []{$\vdots$}; &
        \node (d22) []{$\vdots$}; &
        \node (d23) []{$\vdots$}; &
        \node (d24) []{$\vdots$}; &
        \node (d25) []{$\vdots$}; &
        \\
    };

    \path[->]
        %(A) edge[thick] (x)	% 

        ;
    \begin{pgfonlayer}{background}
        \node [background,
                    fit=(r-1_1) (r-1_5)] {};
        \node [background,
                    fit=(r+1_1) (r+1_5)] {};
    \end{pgfonlayer}
\end{tikzpicture}

